A fourth derivative test for exponential sums

We give an upper bound for the exponential $\sum_{m=1}^M \exp( 2i\pi f (m))$ in terms of $M$ and $\lambda$, where $\lambda$ is a small positive number which denotes the size of the fourth derivative of the real valued function $f$. The classical van der Corput's exponent 1/14 is improved into 1/13 by reducing the problem to a mean square value theorem for triple exponential sums.

==> CrayolaColors.tex <==
% "Crayola" color definitions for Textures 1.7,
% originally due to Tomas Rokick for his dvips definitions.
% Ancient legends have it that these are due to an evening
% spent with "the" 64-color box of Crayola crayons.

% PANTONE color "equivalents" are wild guesses,
% not in any way related to or approved by the
% PANTONE Matching System owners.

\def\GreenYellow{\special{color cmyk 0.15 0 0.69 0}} % PANTONE 388
\def\Yellow{\special{color cmyk 0 0 1. 0}} % PANTONE YELLOW
\def\Goldenrod{\special{color cmyk  0 0.10 0.84 0}} % PANTONE 109
\def\Dandelion{\special{color cmyk 0 0.29 0.84 0}} % PANTONE 123
\def\Apricot{\special{color cmyk 0 0.32 0.52 0}} % PANTONE 1565
\def\Peach{\special{color cmyk 0 0.50 0.70 0}} % PANTONE 164
\def\Melon{\special{color cmyk 0 0.46 0.50 0}} % PANTONE 177
\def\YellowOrange{\special{color cmyk 0 0.42 1. 0}} % PANTONE 130
\def\Orange{\special{color cmyk 0 0.61 0.87 0}} % PANTONE ORANGE-021
\def\BurntOrange{\special{color cmyk 0 0.51 1. 0}} % PANTONE 388
\def\Bittersweet{\special{color cmyk 0 0.75 1. 0.24}} % PANTONE 167
\def\RedOrange{\special{color cmyk 0 0.77 0.87 0}} % PANTONE 179
\def\Mahogany{\special{color cmyk 0 0.85 0.87 0.35}} % PANTONE 484
\def\Maroon{\special{color cmyk 0 0.87 0.68 0.32}} % PANTONE 201
\def\BrickRed{\special{color cmyk 0 0.89 0.94 0.28}} % PANTONE 1805
\def\Red{\special{color cmyk 0 1. 1. 0}} % PANTONE RED
\def\OrangeRed{\special{color cmyk 0 1. 0.50 0}} % No PANTONE match
\def\RubineRed{\special{color cmyk 0 1. 0.13 0}} % PANTONE RUBINE-RED
\def\WildStrawberry{\special{color cmyk 0 0.96 0.39 0}} % PANTONE 206
\def\Salmon{\special{color cmyk 0 0.53 0.38 0}} % PANTONE 183
\def\CarnationPink{\special{color cmyk 0 0.63 0 0}} % PANTONE 218
\def\Magenta{\special{color cmyk 0 1. 0 0}} % PANTONE PROCESS-MAGENTA
\def\VioletRed{\special{color cmyk 0 0.81 0 0}} % PANTONE 219
\def\Rhodamine{\special{color cmyk 0 0.82 0 0}} % PANTONE RHODAMINE-RED
\def\Mulberry{\special{color cmyk 0.34 0.90 0 0.02}} % PANTONE 241
\def\RedViolet{\special{color cmyk 0.07 0.90 0 0.34}} % PANTONE 234
\def\Fuchsia{\special{color cmyk 0.47 0.91 0 0.08}} % PANTONE 248
\def\Lavender{\special{color cmyk 0 0.48 0 0}} % PANTONE 223
\def\Thistle{\special{color cmyk 0.12 0.59 0 0}} % PANTONE 245
\def\Orchid{\special{color cmyk 0.32 0.64 0 0}} % PANTONE 252
\def\DarkOrchid{\special{color cmyk 0.40 0.80 0.20 0}} %  No PANTONE match
\def\Purple{\special{color cmyk 0.45 0.86 0 0}} % PANTONE PURPLE
\def\Plum{\special{color cmyk  0.50 1. 0 0}} % PANTONE 518
\def\Violet{\special{color cmyk 0.79 0.88 0 0}} % PANTONE VIOLET
\def\RoyalPurple{\special{color cmyk 0.75 0.90 0 0}} % PANTONE 267
\def\BlueViolet{\special{color cmyk 0.86 0.91 0 0.04}} % PANTONE 2755
\def\Periwinkle{\special{color cmyk 0.57 0.55 0 0}} % PANTONE 2715
\def\CadetBlue{\special{color cmyk 0.62 0.57 0.23 0}} % PANTONE (534+535)
\def\CornflowerBlue{\special{color cmyk 0.65 0.13 0 0}} % PANTONE 292
\def\MidnightBlue{\special{color cmyk 0.98 0.13 0 0.43}} % PANTONE 302
\def\NavyBlue{\special{color cmyk 0.94 0.54 0 0}} % PANTONE 293
\def\RoyalBlue{\special{color cmyk 1. 0.50 0 0}} % No PANTONE match
\def\Blue{\special{color cmyk 1. 1. 0 0}} % PANTONE BLUE-072
\def\Cerulean{\special{color cmyk 0.94 0.11 0 0}} % PANTONE 3005
\def\Cyan{\special{color cmyk 1. 0 0 0}} % PANTONE PROCESS-CYAN
\def\ProcessBlue{\special{color cmyk 0.96 0 0 0}} % PANTONE PROCESS-BLUE
\def\SkyBlue{\special{color cmyk 0.62 0 0.12 0}} % PANTONE 2985
\def\Turquoise{\special{color cmyk 0.85 0 0.20 0}} % PANTONE (312+313)
\def\TealBlue{\special{color cmyk 0.86 0 0.34 0.02}} % PANTONE 3145
\def\Aquamarine{\special{color cmyk 0.82 0 0.30 0}} % PANTONE 3135
\def\BlueGreen{\special{color cmyk 0.85 0 0.33 0}} % PANTONE 320
\def\Emerald{\special{color cmyk 1. 0 0.50 0}} % No PANTONE match
\def\JungleGreen{\special{color cmyk 0.99 0 0.52 0}} % PANTONE 328
\def\SeaGreen{\special{color cmyk 0.69 0 0.50 0}} % PANTONE 3268
\def\Green{\special{color cmyk 1. 0 1. 0}} % PANTONE GREEN
\def\ForestGreen{\special{color cmyk 0.91 0 0.88 0.12}} % PANTONE 349
\def\PineGreen{\special{color cmyk 0.92 0 0.59 0.25}} % PANTONE 323
\def\LimeGreen{\special{color cmyk 0.50 0 1. 0}} % No PANTONE match
\def\YellowGreen{\special{color cmyk 0.44 0 0.74 0}} % PANTONE 375
\def\SpringGreen{\special{color cmyk 0.26 0 0.76 0}} % PANTONE 381
\def\OliveGreen{\special{color cmyk 0.64 0 0.95 0.40}} % PANTONE 582
\def\RawSienna {\special{color cmyk 0 0.72 1. 0.45}} % PANTONE 154
\def\Sepia{\special{color cmyk 0 0.83 1. 0.70}} % PANTONE 161
\def\Brown{\special{color cmyk 0 0.81 1. 0.60}} % PANTONE 1615
\def\Tan{\special{color cmyk 0.14 0.42 0.56 0}} % No PANTONE match
\def\Gray{\special{color cmyk 0 0 0 0.50}} % PANTONE COOL-GRAY-8
\def\Black{\special{color cmyk 0 0 0 1.}} % PANTONE PROCESS-BLACK
\def\White{\special{color cmyk 0 0 0 0}} % No PANTONE match

\def\BleuIECN{\special{color cmyk 0.98 0.13 0 0.55}}

==> option_keys.tex <==
\ifx\optionkeymacros\undefined\else\endinput\fi
% This document is in the Public Domain.
% It was created by Doug Henderson, Blue Sky Research,
% with modifications suggested by Joseph C. Várilly.
% Added single quotes on 6-4-93.
%
% option_keys - 6-4-93 (last modification)
%
% This macro set defines characters found in the Apple Macintosh
% Monaco font. They allow users to simply type the keystroke
% equivalent of the character desired, such as ø, and have Textures
% typeset it correctly, substituting the TeX macro equivalent
% for the character.
%
% The reason for the creation of this macro set was to take
% advantage of Knuth's new TeX 3.0 capabilities with 8-bit character
% sets. This functionality has been included in our Textures as
% of version 1.3. By typing in nearly any character from the
% Macintosh keyboard, you can typeset with the characters directly
% rather than needing to define macros for these diacritic characters.
% Remember: these just expand single characters. They may not be
% defined in every context or mode.
%
% There are two sections to the macros; the first contains
% characters which can be rendered by depressing the option key
% and another key or shift and option keys with another key,
% and secondly, a combination of various keystrokes together
% to obtain the desired character. For example,
% to create the ø character, you depress the option and o character
% at the same time; to create the uppercase version of Ø, you
% hold the shift, option key, and o key down, and to create the
% Ñ character, you first depress the option and n characters,
% then next the shift and n characters. The option and n create
% the tilde character, and the shift n produce the N character.
%
% Math symbols and math operators need special attention.
% When typing in math symbols the same
% rules apply for math mode as before, namely, you must place dollar
% signs or double-dollar signs around these symbols. When typing
% in math operators, such as the square root symbol, TeX expects
% you to supply an argument following it. For example, if you
% would like to take advantage of the definition here for the
% plus-minus sign, ±, and would like to type it directly for use
% in your text, you need to make sure you are in math mode when
% you call for the character, or simply place dollar signs around
% it to print only the plus minus sign thusly, $±$. Similarly,
% you also need to be in math mode when asking for the square root
% symbol, ˆ, and additionally supply an argument to it.
% The following example shows how to use both the plus-minus sign
% and the square root sign in an equation that has been simplified
% for you via these macro definitions.
%      $$-b±ˆ{b^2-4ac}\over{2a}$$

% define the macintosh "option" generated characters

\catcode`\å=\active\defå{{\aa}}       % option a
\catcode`\†=\active\def†{\int}        % option b (math mode)
\catcode`\ç=\active\defç{\c c}        % option c
\catcode`\=\active\def{\partial}    % option d (math mode)
\catcode`\Ÿ=\active\defŸ{\oint}       % option f (math mode) ?
\catcode`\=\active\def{\triangle}   % option j (math mode)
\catcode`\¬=\active\def¬{\neg}        % option l (math mode)
\catcode`\µ=\active\defµ{\mu}         % option m (math mode)
\catcode`\ø=\active\defø{{\o}}        % option o
\catcode`\¼=\active\def¼{\pi}         % option p (math mode w/ arg.)
\catcode`\¦=\active\def¦{{\oe}}       % option q
\catcode`\ß=\active\defß{{\ss}}       % option s
\catcode`\Ý=\active\defÝ{\dagger}     % option t  (math mode)
\catcode`\ˆ=\active\defˆ{\sqrt}       % option v (math mode w/ arg.)
\catcode`\…=\active\def…{\Sigma}      % option w (math mode)
\catcode`\‰=\active\def‰{\approx}     % option x (math mode)
\catcode`\‡=\active\def‡{\Omega}      % option z (math mode)
\catcode`\£=\active\def£{{\it\$}}     % option 3 ($ from italic font)
\catcode`\ƒ=\active\defƒ{\infty}      % option 5 (math mode)
\catcode`\§=\active\def§{{\S}}        % option 6
\catcode`\¶=\active\def¶{{\P}}        % option 7
\catcode`\€=\active\def€{\bullet}     % option 8
\catcode`\ª=\active\defª{\leavevmode\raise.585ex\hbox{\b a}}      % option 9
\catcode`\º=\active\defº{\leavevmode\raise.6ex\hbox{\b o}}        % option 0
\catcode`\'=\active\def'{\not=}       % option = (math mode)
\catcode`\¾=\active\def¾{\leq}        % option , (math mode)
\catcode`\"=\active\def"{\geq}        % option . (math mode)
\catcode`\÷=\active\def÷{\div}        % option / (math mode)
\catcode`\Š=\active\defŠ{{\dots}}     % option ;
\catcode`\æ=\active\defæ{{\ae}}       % option '
\catcode`\«=\active\def«{\og}         % option \ (math mode)
\catcode`\³=\active\def³{``}          % option [
\catcode`\¡=\active\def¡{!`}          % option !
\catcode`\¢=\active\def¢{\rlap/c}     % option 4
\catcode`\Œ=\active\defŒ{`}           % option ]
\catcode`\¹=\active\def¹{'}           % shift option ]

% macintosh "shift-option" generated characters

\catcode`\Å=\active\defÅ{{\AA}}       % shift-option A
\catcode`\Ç=\active\defÇ{\c C}        % shift-option C
\catcode`\Ø=\active\defØ{{\O}}        % shift-option O
\catcode`\½=\active\def½{\Pi}         % shift-option P (math mode)
\catcode`\'=\active\def'{{\OE}}       % shift-option Q
\catcode`\Æ=\active\defÆ{{\AE}}       % shift-option '
\catcode`\×=\active\def×{\diamond}    % shift-option V (math mode)
\catcode`\°=\active\def°{\accent'27}  % shift-option 8
\catcode`\²=\active\def²{''}          % shift-option [
\catcode`\±=\active\def±{\pm}         % shift-option = (math mode)
\catcode`\»=\active\def»{\fg}         % shift-option \ (math mode)
\catcode`\¿=\active\def¿{?`}          % shift-option /
\catcode`\­=\active\def­{--}          % option - (en-dash)
\catcode`\‹=\active\def‹{---}         % shift-option - (em-dash)

% define the macintosh "composite" characters

\catcode`\ä=\active\defä{\"a}        % option u, then  a
\catcode`\ë=\active\defë{\"e}        % option u, then  e
\catcode`\ï=\active\defï{\"{\i}}     % option u, then  i
\catcode`\ö=\active\defö{\"o}        % option u, then  o
\catcode`\ü=\active\defü{\"u}        % option u, then  u
\catcode`\ÿ=\active\defÿ{\"y}        % option u, then  y
\catcode`\Â=\active\defÂ{\^A}        %  ^, then  A
\catcode`\Ä=\active\defÄ{\"A}        % option u, then  A
\catcode`\Ö=\active\defÖ{\"O}        % option u, then  O
\catcode`\Ü=\active\defÜ{\"U}        % option u, then  U
\catcode`\á=\active\defá{\'a}        % option e, then  a
\catcode`\é=\active\defé{\'e}        % option e, then  e
\catcode`\í=\active\defí{\'{\i}}     % option e, then  i
\catcode`\ó=\active\defó{\'o}        % option e, then  o
\catcode`\ú=\active\defú{\'u}        % option e, then  u
\catcode`\É=\active\defÉ{\'E}        % option e, then  E
\catcode`\Ê=\active\defÊ{\^E}        %  ^, then  E
\catcode`\à=\active\defà{\`a}        % option `, then  a
\catcode`\è=\active\defè{\`e}        % option `, then  e
\catcode`\ì=\active\defì{\`{\i}}     % option `, then  i
\catcode`\ò=\active\defò{\`o}        % option `, then  o
\catcode`\ù=\active\defù{\`u}        % option `, then  u
\catcode`\À=\active\defÀ{\`A}        % option `, then  A
\catcode`\ã=\active\defã{\~a}        % option n, then  a
\catcode`\ñ=\active\defñ{\~n}        % option n, then  n
\catcode`\õ=\active\defõ{\~o}        % option n, then  o
\catcode`\Ã=\active\defÃ{\~A}        % option n, then  A
\catcode`\Ñ=\active\defÑ{\~N}        % option n, then  N
\catcode`\Õ=\active\defÕ{\~O}        % option n, then  O
\catcode`\â=\active\defâ{\^a}        % option i, then  a
\catcode`\ê=\active\defê{\^e}        % option i, then  e
\catcode`\î=\active\defî{\^{\i}}     % option i, then  i
\catcode`\ô=\active\defô{\^o}        % option i, then  o
\catcode`\û=\active\defû{\^u}        % option i, then  u

\let\optionkeymacros\null
